Marsellus: A Heterogeneous RISC-V AI-IoT End-Node SoC with 2-to-8b DNN Acceleration and 30%-Boost Adaptive Body Biasing

Emerging Artificial Intelligence-enabled Internet-of-Things (AI-IoT) System-on-a-Chip (SoC) for augmented reality, personalized healthcare, and nano-robotics need to run many diverse tasks within a power envelope of a few tens of mW over a wide range of operating conditions: compute-intensive but strongly quantized Deep Neural Network (DNN) inference, as well as signal processing and control requiring high-precision floating-point. We present Marsellus, an all-digital heterogeneous SoC for AI-IoT end-nodes fabricated in GlobalFoundries 22nm FDX that combines 1) a general-purpose cluster of 16 RISC-V Digital Signal Processing (DSP) cores attuned for the execution of a diverse range of workloads exploiting 4-bit and 2-bit arithmetic extensions (XpulpNN), combined with fused MAC&LOAD operations and floating-point support; 2) a 2-8bit Reconfigurable Binary Engine (RBE) to accelerate 3x3 and 1x1 (pointwise) convolutions in DNNs; 3) a set of On-Chip Monitoring (OCM) blocks connected to an Adaptive Body Biasing (ABB) generator and a hardware control loop, enabling on-the-fly adaptation of transistor threshold voltages. Marsellus achieves up to 180 Gop/s or 3.32 Top/s/W on 2-bit precision arithmetic in software, and up to 637 Gop/s or 12.4 Top/s/W on hardware-accelerated DNN layers.

==> tables/rbe_related_work.tex <==
\begin{table*}[tbp]
  \centering
  \caption{Comparison of \rbe{} with related work.}
  % \begin{adjustbox}{width=1.5\textwidth,totalheight=\textheight,keepaspectratio}
  % \small{
  \begin{threeparttable}
    \begin{tabular}{@{}lllllll@{}}
      \toprule
        & \rbe{}~\cite{conti2023marsellus}   & Envision~\cite{moons2017envision}
        & UNPU~\cite{Lee2019}             & ISSCC2020~\cite{lin20207}
        & ISSCC2020~\cite{jiao20207}      & BitBlade~\cite{ryu2022bitblade} \\
      \midrule
      % \multirow{1}{*}{Type}
      %   & \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}} Si \end{tabular}}
      %   & \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}} Si \end{tabular}}
      %   & \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}} Si \end{tabular}}
      %   & \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}} Si \end{tabular}}
      %   & \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}} Si \end{tabular}}
      %   & \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}} Si \end{tabular}} \\
      Technology      & 22nm FDX    & 28nm FD-SOI   & 65nm CMOS   & 7nm         & TSMC 12nm   & 28nm        \\
      Area            & 0.13 mm$^2$ & 1.87mm$^2$    & 13.18mm$^2$ & 3.04mm$^2$  & 709mm$^2$   & 0.71mm$^2$  \\
      \multirow{1}{*}{SRAM}
        & \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}} 128 KB L1 \end{tabular}}
        & \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}} 144   KB \end{tabular}}
        & \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}} 256   KB \end{tabular}}
        & \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}} 2176  KB \end{tabular}}
        & \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}} 384   KB \end{tabular}}
        & \multirow{1}{*}{\begin{tabular}[c]{@{}l@{}} 144   KB \end{tabular}} \\
      \midrule
      A bits & 2-8 bit     & 4, 8, 16 bit  & 16 bit      & 8, 16 bit   & 8, 16 bit   & 2, 4, 8 bit  \\
      W bits & 2-8 bit     &               & 1-16 bit    & 8, 16 bit   & 8, 16 bit   & 2, 4, 8 bit  \\
      \midrule
      \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\#Mul \\ Type of Mul \end{tabular}}
        & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} 10'368 \\ 1b\x{}1b MULs \end{tabular}}
        & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} 4'096  \\ 4b\x{}4b MULs \end{tabular}}
        & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} 18'432 \\ 16b\x{}1b Acc \end{tabular}}
        & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} - \end{tabular}}
        & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} - \end{tabular}}
        & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} 4'096 \\ 2b\x{}2b MULs \end{tabular}} \\ \\
      \midrule
      Frequency & 100-420MHz  & 200MHz @1.0V  & 5-200MHz  & 290-880MHz    & 475-700MHz  & 44-195MHz  \\
      Voltage   & 0.5-0.8V    & 0.6-1.0V      & 0.63-1.1V & 0.575-0.825V  & -           & 0.6-1.0V   \\
      \midrule
      \multirow{3}{*}{Peak Perf}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 0.637 TOp/s \\ (2b\x{}2b,  \\ 0.8V+ABB)\end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 0.41  TOp/s \\ (4b\x{}4b,  \\ 1.0V) \end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 7.37  TOp/s \\ (16b\x{}1b, \\ 1.1V) \end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 3.604 TOp/s \\ (8b\x{}8b,  \\ 0.83V) \end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 825   TOp/s \\ (8b\x{}8b) \end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 1.42  TOp/s \\ (2b\x{}2b,  \\ 1.0V) \end{tabular}} \\ \\ \\
      \midrule
      \multirow{3}{*}{Peak Area Eff}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 4.9   TOp/s/mm$^2$ \\ (2b\x{}2b,  \\ 0.8V+ABB)\end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 0.22  TOp/s/mm$^2$ \\ (4b\x{}4b,  \\ 1.0V) \end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 0.56  TOp/s/mm$^2$ \\ (16b\x{}1b, \\ 1.1V) \end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 1.19  TOp/s/mm$^2$ \\ (8b\x{}8b,  \\ 0.83V) \end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 1.16  TOp/s/mm$^2$ \\ (8b\x{}8b) \end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 2.0   TOp/s/mm$^2$ \\ (2b\x{}2b,  \\ 1.0V) \end{tabular}} \\ \\ \\
      \midrule
      \multirow{3}{*}{Energy Eff}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 12.4  TOp/s/W \\ (2b\x{}2b,  \\ 0.8V)\end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 4.3   TOp/s/W \\ (4b\x{}4b,  \\ 1.0V) \end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 50.6  TOp/s/W \\ (16b\x{}1b, \\ 0.66V) \end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 6.83  TOp/s/W \\ (8b\x{}8b,  \\ 0.83V) \end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 2.95  TOp/s/W \\ (8b\x{}8b) \end{tabular}}
        & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} 44.1  TOp/s/W \\ (2b\x{}2b,  \\ 0.6V) \end{tabular}} \\ \\ \\
      \bottomrule
    \end{tabular}
    % \begin{tablenotes}[para, flushleft]
    %     \item [a] 8x64 tensor cores
    %     \item [b] power: core-only
    %     \item [c] complete system area / core-only area
    % \end{tablenotes}
  \label{tab:rbe:rbe_rel_work}
  \end{threeparttable}
  % }
  % \end{adjustbox}
\end{table*}
